Gibbs measures on Subshifts

The notion of Gibbs Measure is used by many researchers of the communities of Mathematical Physics, Probability, Thermodynamic Formalism, Symbolic Dynamics, and others. A natural question is when these several different notions of Gibbs measure coincide. We study the properties of Gibbs measures for functions with $d-$summable variation defined on a subshift $X$. Based on Meyerovitch's work, we prove that if $X$ is a subshift of finite type (SFT), then any equilibrium measure is also a Gibbs measure. Although the definition provided by Meyerovitch does not make any mention to conditional expectations, we show that in the case where $X$ is a SFT, it is possible to characterize these measures in terms of more familiar notions presented in the literature of Mathematical Physics using DLR equations.

==> Makefile <==
# 
# makefile para a compilação do documento
#
# Sáb Jun 23 21:13:37 BRT 2007
#

BASE_NAME = tese-exemplo

LATEX     = latex
PDFLATEX  = pdflatex
BIBTEX    = bibtex
MAKEINDEX = makeindex

pdf: $(BASE_NAME).pdf
ps: $(BASE_NAME).ps

$(BASE_NAME).pdf: $(BASE_NAME).tex 
	$(PDFLATEX) $<
	$(BIBTEX) $(BASE_NAME) 
	$(MAKEINDEX) $(BASE_NAME) 
	$(PDFLATEX) $< 
	$(PDFLATEX) $<
	$(PDFLATEX) $<

$(BASE_NAME).ps: $(BASE_NAME).tex 
	$(LATEX) $<
	$(BIBTEX) $(BASE_NAME) 
	$(MAKEINDEX) $(BASE_NAME) 
	$(LATEX) $< 
	$(LATEX) $<
	$(LATEX) $<
	
clean:
	rm -f $(BASE_NAME)*.ps $(BASE_NAME)*.dvi *.log \
	      *.aux *.blg *.toc *.brf *.ilg *.ind \
	      missfont.log $(BASE_NAME)*.bbl $(BASE_NAME)*.pdf $(BASE_NAME)*.out \
		  $(BASE_NAME)*.lof $(BASE_NAME)*.lot 


==> ape-FM.tex <==
\chapter{Appendix for Chapter 1}
\label{cap:FM}

\section{Feldman-Moore Theorem}\label{secfm}

First, lets present an important auxiliary result due to Feldman and Moore \cite{feldman:77}. Note that
this result is closely related to the Example \ref{group} on Chapter \ref{cap:res}.

\begin{teo}[Feldman and Moore]\label{fmteo}
Let $\mathcal{R}$ a countable standard equivalence relation on a Polish space $X$. Then exists a countable group
$G \subseteq \textsf{Aut(}X\textsf{)}$ such that $\mathcal{R} = \mathcal{R}_G$.
\end{teo}

\begin{proof}

\end{proof}

\section{Radon-Nikodym derivatives}

From now on, we work on the same setting as in Chapter \ref{cap:res}, where $\mathcal{R}$ is a countable equivalence relation
on a Polish space $X$ and $\mu$ a $\sigma$-finite Borel measure quasi-invariant for $\mathcal{R}$. Also, we denote by $\mathcal{C}$ the restriction of $\mathcal{B}(X \times X)$ to $\mathcal{R}$, i.e.,
$\mathcal{C} = \{B\cap \mathcal{R} : B \in \mathcal{B}(X \times X)\} = \{B \in \mathcal{B}(X \times X) : B \subseteq \mathcal {R}\}$.

\begin{prop}
For all $C \in \mathcal{C}$, $\mu(\pi_1(C)) = 0 \iff \mu(\pi_2(C))$.
\end{prop} 

\begin{proof}

\end{proof}

We say that two measures $\nu_1$ and $\nu_2$ on $X$ are equivalent, and denote this fact by $\nu_1 \sim \nu_2$, if : 
$\nu_1 \ll \nu_2$ and $\nu_2 \ll \nu _1$. In other words, $\nu_1 \sim \nu_2$ if, and only if, the null sets of $\nu_1$ and
$\nu_2$ are the same.

\begin{teo}
The following properties holds
\begin{description}
\item[](a) For all $C \in \mathcal{C}$, the map $X \ni x \mapsto |\pi_{1}^{-1}(\{x\})\cap X|$ is Borel-measurable and the following measure
\begin{equation}
\nu_1(C) \defeq \int{|\pi_{1}^{-1}(\{x\}) \cap C|\, d\mu (x)} 
\end{equation}
is $\sigma$-finite, and will be called the left counting measure of $\mu$.

\item[](b) The null sets of $\nu_1$ are exately the elements of $\{C \in \mathcal{C}: \mu(\pi_1(C)) = 0\}$.

\item[](c) For all $C \in \mathcal{C}$, the map $X \ni x \mapsto |\pi_{2}^{-1}(\{x\})\cap X|$ is Borel-measurable and the following measure
\begin{equation}
\nu_2(C) \defeq \int_{X}{|\pi_{2}^{-1}(\{x\}) \cap C|\, d\mu (x)} 
\end{equation}
is $\sigma$-finite, and will be called the right counting measure of $\mu$.

\item[] (d) We have $\nu_2 = \nu_2 \circ \theta$ and $\nu_1 \sim \nu_2$.
\end{description}
\end{teo}

\begin{proof}

\end{proof}

\begin{mydef}
The Radon-Nikodym derivative of $\mu$ with respect to $\mathcal{R}$ is the Borel function $D = D_{\mu,\mathcal{R}} : \mathcal{R} \rightarrow (0,+\infty)$ given by
\begin{equation}
D(x,y) = \frac{d\nu_1}{d\nu_2}(x,y) \qquad, \forall (x,y) \in \mathcal{R}.
\end{equation}
This function is unique up to null sets of $\nu_1$ (or $\nu_2$).
\end{mydef}

\begin{mydef}
A partial Borel isomorphism on $X$ is a Borel isomorphism $f : A \rightarrow B$, where $A, B \in \mathcal{B}$. 
\end{mydef}

\begin{prop}
For every partial Borel isomorphism $f : A \rightarrow B$ with $\textnormal{gr}(f) \subseteq \mathcal{R}$, then $f_{\ast}\mu$ is absolutely continuous with respect
to $\mu$ (viewed as a measure on B) and 
\begin{equation}
\frac{d(f_{\ast}\mu)}{d\mu}(y) = D\big(f^{-1}(y),y\big) \qquad, \; \text{for} \;\mu\text{-a.e}\;\, y \in B.
\end{equation}
\end{prop}


==> ape-eita.tex <==
\chapter{Generators for $\mathcal{F}(X)$}
\label{ape2}

\section{Permutations}\label{pi}

Let $\Omega \neq \emptyset$ be a finite set and $\mathsf{Sym(}\Omega{)}$ the group of all permutations on $\Omega$. Given $\pi \in \mathsf{Sym(}\Omega{)}$ and $x \in \Omega$, define
\[\text{orb}_{\pi}(x) \defeq \big\{\pi^jx: j\geq 0\big\}\]

\begin{lemma}
For any $\pi \in \mathsf{Sym(}\Omega{)}$ and $x \in \Omega$, exists $n \in \mathbb{N}$ such that $\pi^nx=x$.
\end{lemma}
\begin{proof}
Let's suppose that for any $n \in \mathbb{N}$ we have $\pi^nx \neq x$. Let's prove by induction that for all $n \in \mathbb{N}$: $\pi^nx \neq \pi^jx$, $0\leq j \leq n-1$.
For $n=1$ it's trivial. Assuming the vality of this statement for $n \in \mathbb{N}$, it follows that
$\pi^{n+1}x = \pi(\pi^nx) \neq \pi(\pi^jx) = \pi^{j+1}x$ for all $0 \leq j \leq n-1$. So, $\pi^{n+1}x \neq \pi^jx$ for all 
$0 \leq j \leq n$. Therefore, $\text{orb}_{\pi}(x)$ is an infinite subset of $\Omega$, a contradiction.
\end{proof}

Define $\tau(x) \defeq \min\{n \in \mathbb{N}:\pi^nx=x\}$ and note that 
\[\text{orb}_{\pi}(x) = \big\{\pi^jx: 0 \leq j \leq \tau(x)-1\big\}\]
furthermore, $\pi^ix \neq \pi^jx$, for any $0 \leq i < j \leq \tau(x)-1$.

\begin{lemma}
Fixed $\pi \in \mathsf{Sym(}\Omega{)}$, it's possible to decompose $\Omega$ in the following manner:
\[\Omega = \bigsqcup\limits_{i=1}^k \text{orb}_{\pi}(x_i)\]
for some $k \in \mathbb{N}$ and $x_i \in \Omega$, $1 \leq i \leq k$.
\end{lemma}

\begin{proof}
First let's show that for all $x,y \in \Omega$, $\text{orb}_{\pi}(x)=\text{orb}_{\pi}(y)$ if, and only if, $\text{orb}_{\pi}(x) \cap \text{orb}_{\pi}(y) \neq \emptyset$.
The first implication is trivial. On the other hand, if exists  $z \in \text{orb}_{\pi}(x) \cap \text{orb}_{\pi}(y)$, 
then exists $0 \leq n \leq \tau(x)-1$ and $0 \leq m \leq \tau(y)-1$ such that $z= \pi^nx = \pi^my$. Therefore,
$x=\pi^{\tau(x)}x = \pi^{\tau(x)-n}(\pi^nx)= \pi^{\tau(x)-n}(\pi^my) = \pi^{\tau(x)-n+m}y \in \text{orb}_{\pi}(y)$. So,
$\text{orb}_{\pi}(x) \subseteq \text{orb}_{\pi}(y)$. The another inclusion is analogous.
Using the fact proved above, 
\[\Omega = \bigcup\limits_{x \in \Omega} \text{orb}_{\pi}(x) = \bigsqcup\limits_{i=1}^k \text{orb}_{\pi}(x_i)\]
for some $k \in \mathbb{N}$ and $x_i \in \Omega$, $0 \leq i \leq k$.
\end{proof}

It follows from the lemma above that every $\pi \in \mathsf{Sym(}\Omega{)}$ can be written as a product of transpositions
in the following form:
\begin{equation}{\label{satanas}}
\pi = \big(\tau_{x_1, \pi^{n_1-1}x_1}  \circ \cdots \circ \tau_{x_1, \pi x_1} \circ \tau_{x_1,x_1}\big) \circ \cdots \circ \big(\tau_{x_k, \pi^{n_k -1}x_k}  \circ \cdots \circ \tau_{x_k, \pi x_k}\circ \tau_{x_k,x_k}\big)
\end{equation}
where $n_i = \tau(x_i)$.

\section{Generators for $\mathcal{F}(X)$}\label{gen}

We obtain below some convenient generators for $\mathcal{F}(X)$.

Given $\Lambda \subseteq \zd$ finite, we say that $a,b \in X_{\Lambda}$ are compatible if for every $x \in X$ we have
$ax_{\Lambda^c} \in X$ if and only if $bx_{\Lambda^c}\in X$. In this case, we denote $a \approx b$. We also introduce a map
$\xi_{a,b} : X \rightarrow X$ given by

\begin{equation}
\xi_{a,b}(x) = 
\begin{cases}
ax_{\Lambda^c} &, \text{if}\; x_{\Lambda} = b; \\
bx_{\Lambda^c} &, \text{if}\; x_{\Lambda} = a; \\
\;\;x &, \text{otherwise}.
\end{cases}
\end{equation} 

If $\tau_{a,b} \in \mathsf{Sym(}X_{\Lambda}\mathsf{)}$ is the permutation which exchange $a$ and $b$ we can express the equation above
simply as $\xi_{a,b}(x) = \tau_{a,b}(x_{\Lambda}) x_{\Lambda^c}$. Then, it's easy to check that $\xi_{a,b}$ is an involution and
belongs to $\mathcal{F}(X)$.

\begin{lemma}{\label{satan}}
$\mathcal{F}(X)$ is generated by 
\begin{equation}\label{invo}
\big\{\xi_{a,b} : a,b \in X_{B_N}\; \text{are compatible}, N \in \mathbb{N}\big\}.
\end{equation}

\end{lemma}

\begin{proof}
Recall that $\mathcal{F}(X) = \bigcup\limits_{N \in \mathbb{N}}\mathcal{F}_N(X)$. 
Then, fixed $N \in \mathbb{N}$, let's show that every $\varphi \in \mathcal{F}_N(X)$ can be written as a product
of involutions like (\ref{invo}).  

\emph{Step 1.}
Note that $\mathcal{F}_N(X)$ is a subgroup of $\mathcal{F}(X)$. Let's define a map $\alpha$ from 
$\mathcal{F}_N(X)$ into $\mathsf{Sym(}X_{B_N}\mathsf{)}$ and show that $\alpha$ is a one-to-one homomorphism.

Define
\begin{eqnarray*}
\alpha : \mathcal{F}_N(X) &\longrightarrow & \mathsf{Sym(}X_{B_N}\mathsf{)} \\
\varphi & \longmapsto & \widetilde{\varphi} 
\end{eqnarray*}
where $\widetilde{\varphi}(a) \defeq \varphi (x)_{B_N}$, for $x \in X$ satisfying $x_{B_{N}} = a$. By property $(b)$, $\widetilde{\varphi}$ is well defined.
Moreover, $\widetilde{\varphi}$ is invertible, and its inverse is $\widetilde{\varphi^{-1}}$.

Now, let's show that $\alpha$ is a one-to-one homomorphism. Let $\varphi,\psi \in \mathcal{F}_N(X)$, then we have
$\alpha(\varphi \circ \psi)(x_{B_N}) = (\varphi \circ \psi)(x)_{B_N}=\varphi\big(\psi (x)\big)_{B_N} = \widetilde{\varphi}\big(\psi (x)_{B_N}\big) = \widetilde{\varphi}\big(\widetilde{\psi}(x_{B_N})\big) =
\big(\widetilde{\varphi}\circ\widetilde{\psi}\big)(x_{B_N}) = \big(\alpha(\varphi)\circ \alpha(\psi)\big)(x_{B_N})$, for all $x \in X$. So, $\alpha(\varphi \circ \psi)=\alpha(\varphi)\circ \alpha(\psi)$.
Given $\varphi,\psi \in \mathcal{F}_N(X)$, $\alpha(\varphi)=\alpha(\psi)$ implies $\varphi (x)_{B_N}=\psi (x)_{B_N}$, for all $x \in X$. Furthermore, by definition, $\varphi (x)_{B_N^c} = x_{B_N^c} = \psi (x)_{B_N^c}$, for all $x \in X$.
So, $\varphi = \psi$.

\emph{Step 2.} For all $a,b \in X_{B_N}$ such that $a \approx b$, define
\begin{eqnarray*}
\xi_{a,b} : X &\longrightarrow& X \\
x &\longmapsto& \tau_{a,b}(x_{B_N})x_{B_N^c}
\end{eqnarray*}
where $\tau_{a,b} \in \mathsf{Sym(}X_{B_N}\mathsf{)}$ is the transposition which exchange $a$ and $b$. Note that $a \approx b$ implies that $\xi_{a,b}(x) \in X$, for all $x \in X$.

%Note that in fact $\xi_{a,b}(x) \in X$: for all $x \in X$,
%\begin{equation*}
%\begin{cases}
% \text{if}\; x_{B_N}=a,\; \text{then}\; ax_{B_N^c} \in X \implies \xi_{a,b}(x)=bx_{B_N^c} \in X; \\
% \text{if}\; x_{B_N}=b,\; \text{then}\; bx_{B_N^c}, \in X \implies \xi_{a,b}(x)=ax_{B_N^c	} \in X; \\
% \text{otherwise},\; \xi_{a,b}(x)=x \in X.
%\end{cases}
%\end{equation*}

Now, let's show that $\xi_{a,b} \in \mathcal{F}_N(X)$. Note that $\xi_{a,b}$ is an involution, since $\xi_{a,b} \circ \xi_{a,b}\,(x) = \tau_{a,b}\big(\xi_{a,b}(x)_{B_N}\big)x_{B_N^c} =
\tau_{a,b}\big(\tau_{a,b}(x_{B_N})\big)x_{B_N^c}=x$, for all $x \in X$. 
Furthermore, $\xi_{a,b}$ is continuous. In fact, let $(x^{(n)})_{n \in \mathbb{N}}$ be a sequence on $X$ converging to
$x \in X$. Given $M \geq N$, take $n_0 \in \mathbb{N}$ such that for all $n \geq n_0$ we have $x^{(n)}_{B_M} = x_{B_M}$. Therefore,
for $n \geq n_0$

\begin{equation*}
\begin{cases}
\xi_{a,b}\big(x^{(n)}\big)_{B_N} = \tau_{a,b}\big(x^{(n)}_{B_N}\big) = \tau_{a,b}(x_{B_N}) = \xi_{a,b}(x)_{B_N} \\
\xi_{a,b}\big(x^{(n)}\big)_{B_M \backslash B_N} = x^{(n)}_{B_M \backslash B_N} = x_{B_M \backslash B_N} = \xi_{a,b}(x)_{B_M \backslash B_N}\\
\end{cases}
\end{equation*}
then, $\xi_{a,b}\big(x^{(n)}\big)_{B_M} = \xi_{a,b}(x)_{B_M}$. Therefore, $\xi_{a,b}\big(x^{(n)}\big) \to \xi_{a,b}(x)$ when $n \to +\infty$.
Since $\xi_{a,b}$ is an involution, then it is a homeomorphism. Furthermore, the following properties are satisfied:

\doublespacing

\begin{itemize}
\item[](i)\,$\forall x \in X, \, \xi_{a,b}(x)_{B_N^c} = x_{B_N^c}$;
\item[](ii)\,$\forall x,y \in X \Big(\xi_{a,b}(x)_{B_N}=\xi_{a,b}(y)_{B_N} \iff \tau_{a,b}(x_{B_N})=\tau_{a,b}(y_{B_N}) \iff x_{B_N}=y_{B_N}\Big)$.
\end{itemize}

\onehalfspacing

\emph{Step 3.}	
Now, given $\varphi \in \mathcal{F}_N(X)$, let $\pi = \widetilde{\varphi} \in \mathsf{Sym(}X_{B_N}{)}$. It's possible to write $\pi$ in the following form
(see Appendix \ref{pi})
\[\pi = \tau_{a_1, \pi^{n_1-1}a_1}  \circ \cdots \circ \tau_{a_1, \pi a_1} \circ \tau_{a_1,a_1} \circ \cdots \circ \tau_{a_k, \pi^{n_k -1}a_k}  \circ \cdots \circ \tau_{a_k, \pi a_k}\circ \tau_{a_k,a_k}\]
for some $k \in \mathbb{N}$ and $a_i \in X_{B_N}$, $1 \leq i \leq k$. It's easy to prove that for all $\psi \in \mathcal{F}_N(X)$, given
$a \in X_{B_N}$ we have $a \approx \widetilde{\psi}(a)$. Then, for any $1 \leq i \leq k$ and $0 \leq j \leq n_i-1$
\[a_i \approx \pi^j(a_i)\]
 
Therefore, we conclude that it's possible to express $\alpha(\varphi)$ in the form
\[\alpha(\varphi) = \tau_{a_1,b_1} \circ \cdots \circ \tau_{a_n,b_n}\]
for some $n \in \mathbb{N}$, where $a_i,b_i \in X_{B_N}$ satisfies $a_i \approx b_i$. Then
\begin{eqnarray*}
\alpha(\varphi) &=&  \alpha(\xi_{a_1,b_1}) \circ \cdots \circ \alpha(\xi_{a_n,b_n}) \\
&=& \alpha(\xi_{a_1,b_1} \circ \cdots \circ \xi_{a_n,b_n}) 
\end{eqnarray*} 
Since $\alpha$ is one-to-one, it follows that $\varphi = \xi_{a_1,b_1} \circ \cdots \circ \xi_{a_n,b_n}$.

\end{proof}


==> ape-ft.tex <==
\chapter{Thermodynamic Formalism}
\label{cap:fm}


==> ape-shifts.tex <==
\chapter{Shifts}
\label{cap:shifts}

This chapter will introduce one of the main objects of study in symbolic dynamics, known as subshifts. First, will be
introduced the idea of a full-shift and its topological properties. Finally, in the last section will be discussed the concept
of subshifts.

From now on, an alphabet designates a finite set $\mathcal{A}$ of symbols. 

\section{Full-Shifts}\label{lero}

\begin{mydef}[Full-Shift]
The $d$-dimensional full-shift over the alphabet $\mathcal{A}$ is defined as $\ds$, i.e.,
the set of all functions $x:\zd \rightarrow \mathcal{A}$.
\end{mydef}

\begin{mydef}[Shift map]
Given $n \in \zd$, the shift map on $\ds$ is defined as the map $\sigma^n : \ds \rightarrow \ds$
given by 
\[\sigma^n x = (x_{m+n})_{m \in \zd} \qquad ,\forall x \in \ds\]
i.e., $\sigma^n x$ is an element of $\ds$ such that
\[(\sigma^n x)_m = x_{m+n} \qquad ,\forall m \in \zd\]
\end{mydef}
Immediately we have the following properties: 

\doublespacing

\begin{fact}\label{eta}
For $\textbf{0} = (0,...,0) \in \zd$, $\sigma^{\bf{0}} = \textnormal{id}$.
\end{fact}

\begin{fact}\label{etaa}
For all $m,n \in \zd$, $\sigma^{m} \circ \sigma^{n} = \sigma^{m+n}$.
\end{fact}
Indeed, $\Big((\sigma^{m} \circ \sigma^{n})x\Big)_k = \Big(\sigma^{m}(\sigma^{n}x)\Big)_k = (\sigma^{n}x)_{k+m} = x_{(k+m)+n} = 
x_{k+(m+n)} = (\sigma^{m+n}x)_k$, 
for all $k \in \zd$ and $x \in \ds$. So, $(\sigma^{m} \circ \sigma^{n})x = \sigma^{m+n}x$, for all $x \in \ds$.

\begin{fact}\label{etaaa}
For all $n \in \zd$, the map $\sigma^{n}$ is invertible and its inverse is $\sigma^{-n}$.
\end{fact}

\onehalfspacing

For all $ x \in \ds$, the restriction of $x$ to a subset $\Lambda \subseteq \zd$ will be denoted by
$x_{\Lambda}$. Also, will be convenient use the concatenation notation, where given $a \in \mathcal{A}^{\Lambda}$ and $b \in \mathcal{A}^{\Lambda^c}$, we denote by
$x=ab$ the element of $\ds$ such that $x_{\Lambda}=a$ and $x_{\Lambda^c}=b$. 

\section{The topology of $\ds$}

Naturally, we consider $\mathcal{A}$ endowed with the discrete topology $\tau=\mathcal{P}(\mathcal{A})$ and then endow $\ds$ with product topology $\tau^{\zd}$, also known as the prodiscrete topology. 
This section is devoted to explore some topological properties of $(\ds,\tau^{\zd})$.

\subsection{$\ds$ is metrizable}

For any $N \in \mathbb{Z}$, we define
$B_N \defeq \{k \in \zd : ||k|| \leq N\}$. Note that if $N < 0$, then $B_{N} = \emptyset$.

Lets define a map $\rho : \ds \times \ds \rightarrow [0,+\infty)$ and then show that $\rho$ is a
metric on $\ds$. Given $x,y \in \ds$, define

\[\rho (x,y) = 
\begin{cases}
2^{-K} \; , \; \text{if} \; x \neq y ,\; \text{where} \; K= \max\Big\{N \in \mathbb{Z} : x_{B_{N}} = y_{B_{N}}\Big\}; \\
0 \quad\; , \; \text{if} \; x=y.
\end{cases}
\]
Note that $\rho$ is well defined. Indeed, for all $x, y \in \ds$ such that 
$x \neq y$, exists $n \in \zd$ such that $x_{n} \neq y_{n}$. We see that the set $\Big\{N \in \mathbb{Z} : x_{B_{N}} = y_{B_{N}}\Big\}$
is nonempty (since every negative integer belongs to it) and bounded above by $||n||$, then it assumes a maximum element on $\mathbb{Z}$.

Now, will be verified that $\rho$ is, in fact, a metric on $\ds$. It's sufficient verify the triangular inequality, since the
other properties follows immediately from the definition. 

For any $x, y, z \in \ds$: in which case where $x=z$ or $y=z$,
it's easy to check that $\rho(x,y) = \rho(x,z) + \rho(z,y)$; otherwise, let $\rho(x,z)=2^{-K}$ and $\rho(z,y)=2^{-L}$. Taking
$M = \min\{K,L\}$, then $n \in {B_{M}} \implies n \in {B_{K}}\; \text{and}\; n \in {B_{L}} \implies x_n=z_n \;\text{and}\; z_n=y_n 
\implies x_n = y_n$. So, $x_{B_{M}}= y_{B_{M}}$. Therefore, $\rho(x,y) \leq 2^{-M} < 2^{-K} + 2^{-L} = \rho(x,z) + \rho(z,y)$.   

At the end we obtained a metric space $\big(\ds, \rho\big)$. 
It will be shown bellow that $\rho$ is compatible with the topology of $\ds$.

\begin{prop}
The space $\big(\ds, \tau^{\zd}\big)$ is metrizable.
\end{prop}

\begin{proof}
Consider the metric $\rho$ introduced above and $\tau_{\rho}$ its induced topology.
For $n \in \zd$ and a subset $A$ of $\mathcal{A}$, let's prove that $\pi_{n}^{-1}(A)$ is open with respect to $\rho$. Take $x \in \pi_{n}^{-1}(A)$
and define $M= ||n||$. For all $y \in B(x,2^{-M})$, it follows $\rho(x,y)<2^{-M} \implies
x_{B_{M}} = y_{B_{M}} \implies y_n= x_n \in A$, i.e., $B(x,2^{-M}) \subseteq \pi_{n}^{-1}(A)$.
Therefore, $\{\pi_{n}^{-1}(A): n \in \zd, \, A \subseteq \mathcal{A}\} \subseteq \tau_{\rho}$ by the definition of
product topology, $\tau^{\zd} \subseteq \tau_{\rho}$.

Reciprocally, given $x \in \ds$ and $\epsilon>0$, take $K \in \mathbb{N}$ such that $2^{-K}< \epsilon$.
Consider $U=\bigcap\limits_{n \in {B_K}}\pi_{n}^{-1}(\{x_n\}) \in \tau^{\zd}$. It follows that $y \in U \implies \forall n \in {B_K}, \, y \in \pi_{n}^{-1}(\{x_n\})
\implies \forall n\in {B_K} , \, y_n=x_n \implies y_{B_K}=x_{B_K} \implies \rho(x,y) \leq 2^{-K} < \epsilon$.
So, we conclude that $x \in U \subseteq B(x,\epsilon)$. Since $\{B(x,\epsilon): x \in \ds, \, \epsilon>0\}$ is a topological basis for
$\tau_{\rho}$, then $\tau_{\rho} \subseteq\tau^{\zd}$.

\end{proof}

\subsection{Convergence in $\ds$}

A sequence $(x^{(n)})_{n \in \mathbb{N}}$ in $\ds$ converges to $x \in \ds$ if, and only if,

\[\forall \epsilon>0,\,\exists n_0 \in \mathbb{N},\,\forall n \in \mathbb{N}\,\big(n \geq n_0 \implies \rho(x^{(n)},x) < \epsilon\big) \iff\]
\[\forall N \in \mathbb{N},\,\exists n_0 \in \mathbb{N},\,\forall n \in \mathbb{N}\,\big(n \geq n_0 \implies \rho(x^{(n)},x) \leq 2^{-N}\big) \iff\]

\[\forall N \geq 0,\,\exists n_0 \in \mathbb{N},\,\forall n \in \mathbb{N}\,\big(n \geq n_0 \implies x^{(n)}_{B_N}=x_{B_N}\big)\]

Therefore, $x^{(n)} \rightarrow x$ if, and only if, for every $d$-retangle ${B_N} \subseteq \zd$, $x^{(n)}_{B_N}$ and $x_{B_N}$ 
coincides for $n$ sufficiently large.

\subsection{$\ds$ is compact}
For some technical proofs, it's convenient use the fact that $\ds$ is compact.
This result is obtained applying the Tychonoff's Theorem, however, also will be presented another proof exploring
the fact that $\ds$ is metrizable.

\begin{teo}\label{compact}
The full-shift $\ds$ is compact.
\end{teo}

\begin{proof}[Proof 1]
Since $\mathcal{A}$ is finite, then $(\mathcal{A}, \tau)$ is compact. Using Tychonoff's Theorem, the result follows.

\end{proof}

\begin{proof}[Proof 2]
Take one sequence $(x^{(n)})_{n \in \mathbb{N}}$ in $\ds$. Let's show that there exists some convergent subsequence.

Lets prove that exists $a_0 \in \mathcal{A}^{B_0}$ such that $\big\{n \in \mathbb{N} : x^{(n)}_{B_0}=a_0\big\}$ is infinite. In fact,
suppose that for all $a_0 \in \mathcal{A}^{B_0}$, $\big\{n \in \mathbb{N} : x^{(n)}_{B_0}=a_0\big\}$ is finite. Then,
$\mathbb{N} = \bigcup\limits_{a \in \mathcal{A}^{B_0}}\big\{n \in \mathbb{N} : x^{(n)}_{B_0}=a\big\}$ is finite, a
contradiction. Therefore, take $S_0 =\big\{n \in \mathbb{N} : x^{(n)}_{B_0}=a_0\big\}$.

For $N \geq 0$, suppose defined $a_0 \in \mathcal{A}^{B_0}, a_1 \in \mathcal{A}^{B_1},\dots,a_N \in \mathcal{A}^{B_N}$ and 
$S_0 \supseteq S_1 \supseteq \dots \supseteq S_N$ infinite sets, where $(a_{k+1})_{B_k} = a_{k}$ and $S_{k+1} = \big\{n \in S_{k} : x^{(n)}_{B_{k+1	}}=a_{k+1}\big\}$, for all
$k=0,1,\dots,N-1$.

Analogously above, exists $a_{N+1} \in \mathcal{A}^{B_{N+1}}$ such that $\big\{n \in S_N : x^{(n)}_{B_{N+1}}=a_{N+1}\big\}$
is infinite. In fact, if for every $a_{N+1} \in \mathcal{A}^{B_{N+1}}$ we have $\big\{n \in S_N : x^{(n)}_{B_{N+1}}=a_{N+1}\big\}$
finite, then $S_N = \bigcup\limits_{a \in \mathcal{A}^{B_{N+1}}}\big\{n \in S_N : x^{(n)}_{B_{N+1}}=a\big\}$
is finite, a contradiction. Therefore, define $S_{N+1} = \big\{n \in S_N : x^{(n)}_{B_{N+1}}=a_{N+1}\big\} \subseteq S_N$. Moreover,
it's easy to check that $(a_{N+1})_{B_{N}} = a_N$.

Therefore, we obtained by induction the families $(a_k)_{k \geq 0}$ and $(S_k)_{k \geq 0}$ with the properties cited above.
Taking $x$ as the element of $\ds$ such that $x_{B_k}=a_k$, for all $k \geq 0$. Fix $n_1 \in S_1$ arbitrarily. For $k \geq 2$, take $n_k \in S_k$ such that
$n_k > n_{k-1}$. So, we obtained a subsequence $(x^{(n_k)})_{k \in \mathbb{N}}$ of $(x^{(n)})_{n \in \mathbb{N}}$. 

Given $M \geq 0$, take $k_0 \geq M$. Thus, for all $k \geq k_0$ we have $n_k \geq k \geq M$, therefore, $x_{B_M}^{(n_k)}= (a_{k})_{B_M}= x_{B_M}$.

\end{proof}

\section{Subshifts}

Finally, will be defined bellow the main object of study in this work.

\begin{mydef}[Subshift]
A subset $X \subseteq \ds$ is called a subshift if it's closed and invariant under translations, i.e.,
$\sigma^{n}(X)=X$ for all $n \in \zd$.
\end{mydef}

Let $X \subseteq \ds$ a subshift and consider $\sigma^n$ the shift map on $\ds$. We denote its restriction to 
$X$ by $ \sigma_{X}^n \defeq {\sigma^{n}\upharpoonright}_X: X \rightarrow X$. Now, we have analogous facts 
as Facts \ref{eta}, \ref{etaa} and \ref{etaaa} presented in the section \ref{lero}.	

\doublespacing

\begin{fact} 
For $\textbf{0} = (0,...,0) \in \zd$, $\sigma_X^{\bf{0}} = \textnormal{id}_X$.
\end{fact}
\begin{fact}\label{eitaa}
For all $m,n \in \zd$, $\sigma_X^{m+n} = \sigma_X^{m} \circ \sigma_X^{n}$.
\end{fact}  
Indeed, for any $x \in X$, $\sigma_X^{m+n}(x) = \sigma^{m+n}x \stackrel{\textbf{Fact \ref{etaa}}}{=} \sigma^{m}(\sigma^{n}x) = \sigma_X^{m}(\sigma_X^n(x)) = (\sigma_X^{m} \circ \sigma_X^{n})(x)$.
\begin{fact}
For all $n \in \zd$, the map $\sigma_X^{n}$ is invertible and its inverse is $\sigma_X^{-n}$.\\
\end{fact}
 
\onehalfspacing
 
\begin{prop}\label{homeo}
Given $n \in \zd$, $\sigma_{X}^{n}$ is a homeomorphism. 
\end{prop}

\begin{proof}
It's sufficient show that $\sigma_X^{n}$ is continuous. Let $(x^{(m)})_{m \in \mathbb{N}}$ a sequence in $X$ converging to $x \in X$. Given $N \geq 0$, taking $M=\max\limits_{k \in B_{N}}||k+n||$,   
exists $m_0 \in \mathbb{N}$ such that for all $m \geq m_0$ we have $x_{B_M}^{(m)}=x_{B_M}$. Therefore, if $m \geq m_0$, then $\sigma_X^{n}(x^{(m)})_{B_N}=\sigma_X^{n}(x)_{B_N}$.

\end{proof}

\subsection{Equivalent Definition}

If $\Lambda$ is a finite subset of $\zd$, a function $f : \Lambda \rightarrow \mathcal{A}$ will be called a pattern on $\Lambda$.
Take a collection $\mathcal{F}$ of patterns\footnote{The patterns in this collection will be referred as forbidden patterns.}, more
precisely, $\mathcal{F} \subseteq \bigcup\limits_{\substack{\Lambda \subseteq \zd \\ |\Lambda| < + \infty}}\mathcal{A}^{\Lambda}$. Then, lets define
\[\mathsf{X}_{\mathcal{F}} \defeq \Big\{x \in \ds: \forall \Lambda \subseteq \zd\, \textnormal{finite},\; \forall n \in \zd,\; (\sigma^nx)_{\Lambda} \notin \mathcal{F} \Big\}\]

The following result will give us an alternative characterization of subshifts and, moreover, will allow us to define the concept of a 
subshift of finite type (SFT).

\begin{teo}
A subset $X \subseteq \ds$ is a subshift if, and only if, it can be written in the form $X = \mathsf{X}_{\mathcal{F}}$, for some
collection $\mathcal{F}$ of forbidden patterns.
\end{teo}

\begin{proof}
Let $X$ a subshift of $\ds$, thus $\ds \backslash X$ is open. We have $x \in \ds \backslash X$ if, and only if, exists $n=n(x) \in \mathbb{N}$ such that $B(x,2^{-(n-1)}) \subseteq \ds \backslash X$.
Note that $B(x,2^{-(n-1)})=\{y \in \ds: \rho(x,y)<2^{-(n-1)}\}=\{y \in \ds: \rho(x,y)\leq 2^{-n}\}
=\big\{y \in \ds: x_{B_n}=y_{B_n}\big\}$. Then, for any $x \in \ds \backslash X$ define 
$f_x = x_{B_{n(x)}}$ and consider $\mathcal{F}=\{f_x : x \in \ds \backslash X\}$. Lets show that $X = \mathsf{X}_{\mathcal{F}}$.

Given $x \in \ds$, we have $x \in \ds \backslash X \iff \exists n \in \mathbb{N}, \; x_{B_n} \in \mathcal{F} \iff \exists \Lambda	 \subseteq \zd \; \text{finite}, \; x_\Lambda \in \mathcal{F}$. Then,
$x \in X  \iff \forall \Lambda \subseteq \zd\; \text{finite}, \; x_\Lambda \notin \mathcal{F}$. Using the translation invariance of $X$, 
$x \in X \iff \forall n \in \zd, \; x \in \sigma^{-n}(X) \iff \forall n \in \zd, \; \sigma^{n}x \in X 
\iff \forall \Lambda \subseteq \zd\; \text{finite}, \;\forall n \in \zd, \; (\sigma^{n}x)_\Lambda \notin \mathcal{F} \iff x \in \mathsf{X}_\mathcal{F}$.

Now, lets prove the reciprocal. Consider a collection $\mathcal{F}$ of patterns and take $X=\mathsf{X}_{\mathcal{F}}$.
For all $m \in \zd$, $x \in \sigma^{-m}(X) \iff \sigma^mx \in X \iff \forall \Lambda \subseteq \zd \; \text{finite}, \; \forall n \in \zd,
\; \sigma^{n}(\sigma^{m}x)_\Lambda = (\sigma^{n+m}x)_\Lambda \notin \mathcal{F} \iff \forall \Lambda \subseteq \zd \; \text{finite}, \; \forall n \in \zd,
\; (\sigma^{n}x)_\Lambda \notin \mathcal{F} \iff x \in X$. Therefore, given $m \in \zd$, we have $\sigma^{-m}(X) = X$, equivalently,
$\sigma^{m}(X)= X$.	

Rest to prove that $X$ is closed. Let $(x^{(k)})_{k \in \mathbb{N}}$ a sequence in $X$ converging to some $x \in \ds$.
For any $\Lambda \subseteq \zd$ finite and $n \in \zd$, take $M \geq 0$ such that $\Lambda \subseteq B_M$. The continuity of $\sigma^{n}$ implies
on the existence of $k \in \mathbb{N}$ such that $(\sigma^{n}x^{(k)})_{B_M}= (\sigma^{n}x)_{B_M}$, therefore, $(\sigma^{n}x)_\Lambda = (\sigma^{n}x^{(k)})_\Lambda \notin \mathcal{F}$. 

\end{proof}

\subsection{Subshifts of Finite Type (SFTs)}


\begin{mydef}[SFT]\label{defsft}
A subset $X \subseteq \ds$ is called a subshift of finite type if it can be written as $X=\mathsf{X}_\mathcal{F}$, for some $\mathcal{F}$ finite.
\end{mydef}

\emph{Remark:} Let $\mathcal{F}$ a finite set of patterns such that $X = \mathsf{X}_{\mathcal{F}}$. Without loss of generality, it can be supposed that
all patterns in $\mathcal{F}$ are defined on the same (finite) subset $\Lambda \subseteq \zd$. Indeed, since $\mathcal{F}$ is finite, it can be taken 
a finite subset $\Lambda \subseteq \zd$ which contains the domains of all patterns in $\mathcal{F}$. Then define  $\widetilde{\mathcal{F}}$ as the 
following (finite) set of patterns on $\Lambda$ 
\[\widetilde{\mathcal{F}} = \big\{a \in \mathcal{A}^\Lambda : \exists f \in \mathcal{F}, a\upharpoonright_{\text{Dom}(f)}=f\big\}\]
It's easy to check that 
$X_{\widetilde{\mathcal{F}}} = X_{\mathcal{F}}$.

Now we will present another equivalent definition of subshifts of finite type frequently presented in other texts. Analogous with
Definition \ref{defsft}, SFTs also can be characterized in terms of a finite number of allowed patterns instead of forbidden patterns.   

\begin{prop}
$X$ is a SFT if, and only if, exists $\Lambda \subseteq \zd$ finite and a set $P$ of patterns on $\Lambda$ such that
\[X  = \big\{x \in \ds : \forall n \in \zd, (\sigma^nx)_\Lambda \in P \big\}\] 
\end{prop}

\begin{proof}
Due to the remark above, $X$ is a SFT if, and only if, exists $\Lambda \subseteq \zd$ finite and a collection $\mathcal{F}$ of patterns 
on $\Lambda$ such that $X=\big\{x \in \ds : \forall n \in \zd , (\sigma^nx)_{\Lambda} \notin \mathcal{F}\big\}$. Then if we 
take $P = \mathcal{A}^{\Lambda}\backslash{\mathcal{F}}$, the first implication follows. The second implication follows taking
$\mathcal{F} = \mathcal{A}^{\Lambda} \backslash {P}$.

\end{proof}

\begin{ex}[Matrix Subshifts]
Let $A_1, \dots, A_d \in {\{0,1\}}^{\mathcal{A}\times\mathcal{A}}$ matrices of $0$'s and $1$'s indexed on $\mathcal{A}\times\mathcal{A}$, called transition matrices. Then,
we define
\[\Sigma_{A_1, \dots,A_d} \defeq \big\{x \in \ds : \forall n \in \zd, \forall i \in \{1, \dots, d\}, A_i(x_n,x_{n+\textbf{e}_i}) = 1 \big\}\]
where $\textbf{e}_i = \underbrace{(0, \dots, 1, \dots, 0)}_{\textnormal{i-th position}} \in \zd$.\\

Therefore, $\Sigma_{A_1, \dots,A_d}$ is a SFT. Indeed, if we take $\Lambda = \{\textbf{0}, \textbf{e}_1, \dots, \textbf{e}_d\}$ and
\[P = \big\{a \in \mathcal{A}^\Lambda : \forall i \in \{1, \dots, d\}, A_i\big(a_{\textbf{0}}, a_{\textbf{e}_i}\big) = 1 \big\}\]
then,
\begin{eqnarray*}
\Sigma_{A_1, \dots,A_d} &=& \big\{x \in \ds : \forall n \in \zd, \forall i \in \{1, \dots, d\}, A_i((\sigma^nx)_{\textbf{0}},(\sigma^nx)_{\textbf{e}_i}) = 1 \big\} \\
&=& \big\{x \in \ds : \forall n \in \zd, (\sigma^nx)_{\Lambda} \in P\big\}
\end{eqnarray*}

\end{ex}

\subsection{Final Comments}\label{comm}

Now, we will link some concepts introduced on Chapter \ref{cap:res} with some elements presented in this chapter.

Note that since $X$ is a closed subset of the compact metric space $\ds$, then $(X,\rho\upharpoonright_{X\times X})$ is also a compact metric space.

Furthermore, follows from Proposition \ref{homeo} and Fact \ref{eitaa} that the shift maps define an action of $\zd$ on $X$ by homeomorphisms. Precisely,
it can be defined a map 
\begin{eqnarray*}
T: \zd &\longrightarrow& \textsf{Homeo(}X\textsf{)} \\
n &\longmapsto& \sigma_X^n
\end{eqnarray*}
which is a homomorphism between the groups $(\zd,+)$ and $\big(\textsf{Homeo(}X\textsf{)}, \circ\big)$. This map
will be referred as a shift action. Note that $T$ is expansive. Indeed, given $x,y \in X$ distinct, exists $i \in \zd$ such that $x_i \neq y_i$. So
$(T^ix)_{\textbf{0}} \neq (T^{i}y)_{\textbf{0}}$, therefore, $\rho(T^ix,T^iy) = 2$.

Then, according to Example \ref{gr} from Chapter \ref{cap:res}, it can be defined the Gibbs relation of $(X,T)$, denoted by $\gr$.
Lets prove that in this case we have
\[\gr = \big\{(x,y) \in X \times X : \exists \Lambda \subseteq \zd\, \text{finite}\, , x_{\Lambda^c} = y_{\Lambda^c}\big\}\]

For $(x,y) \in \gr$, exists $N \in \mathbb{N}$ such that for all $k \in \zd$ such that $||k|| > N$ we have $\rho(T^kx,T^ky) \leq 1 = 2^0$, in other words, $x_k = y_k$.
On the other hand, consider $(x,y) \in X\times X$ such that exists $\Lambda \subseteq \zd$ with $x_{\Lambda^c} = y_{\Lambda^c}$. Without loss of generality, it can be supposed
that $\Lambda = B_N$, for some $N \in \mathbb{N}$. Then, given $M \geq 0$, for all $k \in \zd$ such that $||k|| > M+N$, we have 
$(T^kx)_{B_M} = (T^ky)_{B_M}$, i.e., $\rho(T^kx,T^ky) \leq 2^{-M}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> fm <==
The Theorem 5.8.11 from \cite{sri:98} guarantees that exists a countable collection of Borel graphs $(G_n)_{n \in \mathbb{N}}$
such that $\mathcal{R} = \bigcup\limits_{n \in \mathbb{N}}G_n$. For each $n \in \mathbb{N}$, since $G_n$ is a graph it's easy to check that $\pi_l\upharpoonright_{G_n}$ and $\pi_r\upharpoonright_{\theta(G_n)}$ are one-to-one.
Since the diagonal $\Delta \subseteq X \times X$ is closed, then exists a countable collection $(U_k\times V_k)_{k \in \mathbb{N}}$ such that
\[X \times X \backslash \Delta = \bigcup\limits_{k \in \mathbb{N}}U_k\times V_k\]
where $U_k, V_k \subseteq X$ are open sets. Note that $U_k \cap V_k = \emptyset$, otherwise, $U_k \times V_k \subseteq \Delta$.	

Define $D_{m,n,k} \defeq G_m \cap \theta(G_n) \cap (U_k\times V_k)$ for each $m,n,k \in \mathbb{N}$.
We also have that $D_{m,n,k}$ is a Borel set, $\pi_l\upharpoonright_{D_{m,n,k}}$ and $\pi_r\upharpoonright_{D_{m,n,k}}$ are one-to-one
and $\pi_l(D_{m,n,k})\cap\pi_r(D_{m,n,k}) = \emptyset$.

Now define $g_{m,n,k} : X \rightarrow X$ in the following way
\[g_{m,n,k}=
\begin{cases}
y , \;\text{if}\; (x,y) \in D_{m,n,k} \; \text{or}\; (y,x) \in D_{m,n,k}; \\
x,\; \text{otherwise}.
\end{cases}
\]

It's easy to see that $g_{m,n,k}$ is well defined since for all $x \in X$,
\[x \in \pi_l(D_{m,n,k}) \iff \exists ! y \in X, (x,y) \in D_{m,n,k}\]
and
\[x	\in \pi_r(D_{m,n,k}) \iff \exists ! y \in X, (y,x) \in D_{m,n,k}.\]

Using the definition of $g_{m,n,k}$ it's easy to check that $g_{m,n,k}^2 = g_{m,n,k}$. Also,

\begin{eqnarray*}
\textnormal{gr}(g_{m,n,k}) &=& \{(x,y) \in X\times X : y=g_{m,n,k}(x)\} \\
&=& \{(x,y) \in X\times X : x \in \pi_l(D_{m,n,k}) \;\text{and}\; y=g_{m,n,k}(x)\} \\
&\cup& \{(x,y) \in X\times X : x \in \pi_r(D_{m,n,k}) \;\text{and}\; y=g_{m,n,k}(x)\}\\
&\cup& \{(x,y) \in X\times X : x \in X\backslash\big(\pi_l(D_{m,n,k})\cup\pi_r(D_{m,n,k})\big) \;\text{and}\; y=g_{m,n,k}(x)\} \\
&=& D_{m,n,k} \cup \theta(D_{m,n,k}) \cup \Big(X\backslash\big(\pi_l(D_{m,n,k})\cup\pi_r(D_{m,n,k})\big)\Big)^2.
\end{eqnarray*}

Note that $g_{m,n,k}$ is measurable, since $\textnormal{gr}(g_{m,n,k})$ is a Borel subset of $X\times X$. Then take 
$G \subseteq \mathsf{Aut(}X\mathsf{)}$ as the group generated by $\{g_{m,n,k} : m,n,k \in \mathbb{N	}\}$.

Finally, we have that $\mathcal{R} = \Delta \cup \bigcup\limits_{m,n,k \in \mathbb{N}}\textnormal{gr}(g_{m,n,k})$.


